When2com: Multi-Agent Perception via Communication Graph Grouping

While significant advances have been made for single-agent perception, many applications require multiple sensing agents and cross-agent communication due to benefits such as coverage and robustness. It is therefore critical to develop frameworks which support multi-agent collaborative perception in a distributed and bandwidth-efficient manner. In this paper, we address the collaborative perception problem, where one agent is required to perform a perception task and can communicate and share information with other agents on the same task. Specifically, we propose a communication framework by learning both to construct communication groups and decide when to communicate. We demonstrate the generalizability of our framework on two different perception tasks and show that it significantly reduces communication bandwidth while maintaining superior performance.

==> figure/Experimental_Cases.tex <==
\begin{figure}[t]
    \vspace{1mm}
    \begin{center}
    \centerline{\includegraphics[width=\linewidth]{./figure/Experimental_Cases.png}}
    \caption{
        \textbf{An example of our constructed communication groups and the corresponding adjacency matrix.} Blue arrow indicates the intra-agent transmission without bandwidth consumption, and red arrow represents the inter-agent transmission with    bandwidth consumption.}
        \label{fig:experimental_cases}

    \end{center}
    \vspace{-6mm}
\end{figure}

==> table/MIMO_case6.tex <==
\begin{table*}
\caption{\textbf{Experimental results on Multiple-Request Multiple-Partial-Support. (Case 6)}}
\label{tab:res_nav_p}
\centering
\begin{tabular}{cccccc}
\toprule
& & & \multicolumn{3}{c}{mIoU }\\
 \cmidrule(lr){4-6} 
& Models & Bandwidth & Noisy & Normal & Avg. \\
\midrule
Upper bound & All Norm & - & 47.9 & 48.37 & 48.14 \\
\midrule
\multirow{5}{*}{ Fully-connected } & CatAll & 4 & 26.86 & 45.27 & 36.07 \\
& AuxAttend & 4 & 26.97 & 51.03 & 39.00 \\
& Compression & 1 & 22.22 & 32.85 & 27.54 \\
& ComNet~\cite{sukhbaatar2016learning} & 4 & 26.56 & 49.07 & 37.82 \\
& TarMac~\cite{das2019tarmac} & 4 & & & 0 \\
\midrule
\multirow{3}{*}{ Distrbuted } & RandCom & 1 & 24.13 & 45.19 & 34.66 \\
& AwsCom & 1 & 26.97 & 50.71 & 38.84 \\
& Ours & 1.75 & 37.72 & 51.98 & 44.85 \\
\midrule
Lower bound & No Com & - & 25.2 & 46.74 & 35.97 \\
\bottomrule
\end{tabular}
\end{table*}





==> table/MIMO_case7.tex <==
\begin{table*}
\caption{\textbf{Experimental results on Mulitple-Request Multiple-Partial-Support. (Case 7)}}
\label{tab:res_nav_p}
\centering
\begin{tabular}{cccccc}
\toprule
\begin{tabular}{cccccc}
& Models & Bandwidth & All & Noisy & Normal \\
\midrule
 & AllNorm & & 47.14 & 47.35 & 46.95 \\
\midrule
\multirow{6}{*}{ Fully-Connected } & CatAll & 4 & 39.28 & 26.25 & 48.73 \\
& AuxAttend & 4 & 38.3 & 24.49 & 48.37 \\
& Compression & 1 & 25.15 & 24.7 & 25.43 \\
& CommNet~\cite{sukhbaatar2016learning} & 4 & & & \\
& TarMac~\cite{das2019tarmac} & 4 & & & \\
& Ours-FC & 4 & & & \\
\midrule
\multirow{3}{*}{ Distributed } & RandCom & 1 & 38.04 & 22.69 & 49.57 \\
& AwsCom & 1 & 38.3 & 24.49 & 48.37 \\
& Ours-G & & & & \\
\midrule
 & NoCom & & 36.67 & 22.96 & 46.33 \\
\bottomrule
\end{tabular}
\end{tabular}
\end{table*}

==> table/when2com_sancheck.tex <==
% \begin{tabular}{ccccccccc}
% & Models & Bandwidth & All samples & Noisy samples & Normal samples & When2Com Acc. & Who2Com Acc. & BIS score \\
% Upper bound & Single Normal image & & 53.08 & 52.65 & 53.37 & & & \\
% \multirow{5}{*}{ Centralized } & CatAll & 4 & 37.54 & 30.86 & 44.1 & & & \\
% & Auxiliary View Attention (w/ msg) & 4 & 42.14 & 38.08 & 46.09 & & & \\
% & Compression & 4 & 33.3 & 28.48 & 37.98 & & & \\
% & Our when2com (centralized) & 4 & 53.19 & 52.02 & 54.21 & & & \\
% & TarMac & & & & & & & \\
% \multirow{4}{*}{ Distrbuted } & Random Selection & 0.8 & 34.89 & 25.12 & 45.06 & 48.46% & 19.32% & \\
% & AlwaysCom & 1 & 34.89 & 26.82 & 43.76 & 49.04% & 13.27% & \\
% & Ours (w/ msg) & 0.492307 & 53.25 & 52.1 & 54.24 & 99.80% & 98.27% & \\
% & Ours (w/o msg) & & & & & & & \\
% Lower bound & Single Degraded image & & 35.22 & 25.94 & 44.63 & & & \\
% \end{tabular}


\begin{table*}
\caption{\textbf{Experimental results on Hidden Target View of When2Com.}}
\label{tab:res_nav_p}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
& Models & Bandwidth & All samples & Noisy samples & Normal samples & When2Com Acc. & Who2Com Acc. & BIS score \\
\midrule
Upper bound & Single Normal image & & 53.08 & 52.65 & 53.37 & & & \\
\midrule
\multirow{5}{*}{ Centralized } & CatAll (cite two body paper?) & 4 & 37.54 & 30.86 & 44.1 & & & \\
& AuxAttention & 4 & 42.14 & 38.08 & 46.09 & & & \\
& Compression & 4 & 33.3 & 28.48 & 37.98 & & & \\
& Ours (centralized) & 4 & 53.19 & 52.02 & 54.21 & & & \\
& TarMac & & & & & & & \\
\midrule
\multirow{4}{*}{ Distrbuted } & Random Selection & 0.8 & 34.89 & 25.12 & 45.06 & 48.46 & 19.32 & \\
& AlwaysCom & 1 & 34.89 & 26.82 & 43.76 & 49.04 & 13.27 & \\
& Ours (w/ msg) & 0.49 & 53.25 & 52.1 & 54.24 & 99.8 & 98.27 & \\
& Ours (w/o msg) [move this one to analysis] & & & & & & & \\
\midrule
Lower bound & Single Degraded image & & 35.22 & 25.94 & 44.63 & & & \\
\bottomrule
\end{tabular}}
\end{table*}
